Answer Candidate Type Selection: Text-to-Text Language Model for Closed Book Question Answering Meets Knowledge Graphs

Pre-trained Text-to-Text Language Models (LMs), such as T5 or BART yield promising results in the Knowledge Graph Question Answering (KGQA) task. However, the capacity of the models is limited and the quality decreases for questions with less popular entities. In this paper, we present a novel approach which works on top of the pre-trained Text-to-Text QA system to address this issue. Our simple yet effective method performs filtering and re-ranking of generated candidates based on their types derived from Wikidata "instance_of" property.

==> tables/res_large_init.tex <==
\begin{table}
    \footnotesize
    \centering
    
    \begin{tabular}{lccc}
        \hline
        \textbf{KGQA Model} & \multicolumn{3}{c}{\textbf{Tuned on}} \\
        \hline
         & --- & \textbf{SQWD} & \textbf{Mintaka}\\
        \hline
    
        \multicolumn{4}{c}{\it SimpleQuestionsWikidata} \\
        \hline
        BART-base & 0 & 16.54 & 7.08 \\
        Ours (BART-base) & 30.38 & \textbf{42.60} & 30.70 \\
        \hdashline
        BART-large & 0 & 16.97 & 3.02 \\
        Ours (BART-large) & 30.42 & \textbf{42.64} & 31.39 \\
        \hdashline
        T5-base & 0 & 21.26 & 6.19 \\
        Ours (T5-base) & 30.47 & \textbf{43.13} & 34.60 \\
        \hdashline
        T5-large & 0 & 22.36 & 9.43 \\
        Ours (T5-large) & 29.88 & \textbf{43.05} & 36.89 \\
        \hdashline
        T5-large-ssm & 0.57 & 23.66 & 5.92 \\
        Ours (T5-large-ssm) & 23.39 & \textbf{47.42} & 36.54 \\
        \hdashline
        T5-large-ssm-nq & 5.12 & 22.52 & 4.34 \\
        Ours (T5-large-ssm-nq) & 35.09 & \textbf{43.88} & 36.39 \\
        \hdashline
        T5-11b-ssm & 1.81 & --- & --- \\
        Ours (T5-11b-ssm) & \textbf{25.84} & --- & --- \\
        \hdashline
        T5-11b-ssm-nq & 10.94 & --- & --- \\
        Ours (T5-11b-ssm-nq) & \textbf{38.51} & --- & --- \\
        
        \hline
        \multicolumn{4}{c}{\it RuBQ (English)} \\
        \hline
        BART-base & 0 & 5.93 & 3.72 \\
        Ours (BART-base) & 9.50 & 11.65 & \textbf{11.72} \\
        \hdashline
        BART-large & 0 & 4.07 & 4.86 \\
        Ours (BART-large) & 9.50 & 12.15 & \textbf{12.79} \\
        \hdashline
        T5-base & 0 & 6.22 & 6.93 \\
        Ours (T5-base) & 9.44 & 14.44 & \textbf{16.58} \\
        \hdashline
        T5-large & 0 & 11.15 & 12.15 \\
        Ours (T5-large) & 9.44 & 18.94 & \textbf{20.51} \\
        \hdashline
        T5-large-ssm & 0.42 & 21.44 & 23.87 \\
        Ours (T5-large-ssm) & 9.72 & 26.02 & \textbf{27.88} \\
        \hdashline
        T5-large-ssm-nq & 18.87 & 17.80 & 19.23 \\
        Ours (T5-large-ssm-nq) & \textbf{27.52} & 25.38 & 26.38 \\
        \hdashline
        T5-11b-ssm & 14.09 & --- & --- \\
        Ours (T5-11b-ssm) & \textbf{20.94} & --- & --- \\
        \hdashline
        T5-11b-ssm-nq & 33.38 & --- & --- \\
        Ours (T5-11b-ssm-nq) & \textbf{38.31} & --- & --- \\

        \hline
        \multicolumn{4}{c}{\it Mintaka (One-hop, English)} \\
        \hline
        BART-base & 0 & 2.06 & 9.12 \\
        Ours (BART-base) & 4.70 & 5.88 & \textbf{10.29} \\
        \hdashline
        BART-large & 0 & 1.76 & 12.65 \\
        Ours (BART-large) & 4.41 & 5.29 & \textbf{15.29} \\
        \hdashline
        T5-base & 0 & 4.41 & 8.24 \\
        Ours (T5-base) & 4.71 & 8.53 & \textbf{10.59} \\
        \hdashline
        T5-large & 0 & 7.06 & 14.41 \\
        Ours (T5-large) & 4.71 & 10.00 & \textbf{15.88} \\
        \hdashline
        T5-large-ssm & 0.50 & 19.71 & 27.65 \\
        Ours (T5-large-ssm) & 6.76 & 18.53 & \textbf{28.24} \\
        \hdashline
        T5-large-ssm-nq & 17.65 & 14.12 & 23.24 \\
        Ours (T5-large-ssm-nq) & 22.94 & 14.12 & \textbf{25.59} \\
        \hdashline
        T5-11b-ssm & 20.88 & --- & --- \\
        Ours (T5-11b-ssm) & \textbf{24.71} & --- & --- \\
        \hdashline
        T5-11b-ssm-nq & 41.76 & --- & --- \\
        Ours (T5-11b-ssm-nq) & \textbf{45.00} & --- & --- \\
        \hline
        
    \end{tabular}
    \caption{Evaluation results on three KGQA datasets (Hit@1 scores): comparing seq2seq models with and without proposed approach tunned on SQWD, Mintaka and pre-trained seq2seq models without tuning for QA.}
    \label{tab:full_results}
\end{table}





==> tables/res_large_upd.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lllllllll}
\hline
\multicolumn{9}{c}{KGQA Model}                                                   \\ \hline
\multicolumn{9}{c}{\textit{SimpleQuestionsWikidata}}                                      \\ \hline
Tuned on         & \textbf{\begin{tabular}[c]{@{}l@{}}BART-base/\\ Ours\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}BART-large/\\ Ours\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}T5-base/\\ Ours\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}T5-large/\\ Ours\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}T5-large-ssm/\\ Ours\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}T5-large-ssm-nq/\\ Ours\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}T5-11b-ssm/\\ Ours\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}T5-11b-ssm-nq/\\ Ours\end{tabular}} \\ \hline
-                & 0/30.38                                                            & 0/30.42                                                             & 0/30.47                                                          & 0/29.88                                                           & 0.57/23.39                                                            & 5.12/35.09                                                               & 1.81/\textbf{25.84}                                                          & 10.94/\textbf{38.51}                                                            \\ \hline
\textbf{SQWD}    & 16.54/\textbf{42.60}                                                        & 16.97/\textbf{42.64}                                                       & 21.26/\textbf{43.13}                                                    & 22.36/\textbf{43.05}                                                       & 23.66/\textbf{47.42}                                                           & 22.52/\textbf{43.88}                                                              & -/-                                                                 & -/-                                                                    \\ \hline
\textbf{Mintaka} & 7.08/30.70                                                         & 3.02/31.39                                                          & 6.19/34.60                                                       & 9.43/36.89                                                        & 5.92/36.54                                                            & 4.34/36.39                                                               & -/-                                                                 & -/-                                                                    \\ \hline
\multicolumn{9}{c}{\textit{RuBQ (English)}}                                                                                               \\ \hline
-                & 0/9.50                                                             & 0/9.50                                                              & 0/9.44                                                           & 0/9.44                                                            & 0.42/9.72                                                             & 18.87/\textbf{27.52}                                                              & 14.09/\textbf{20.94}                                                         & 33.38/\textbf{38.31}                                                            \\ \hline
\textbf{SQWD}    & 5.93/11.65                                                         & 4.07/12.15                                                          & 6.22/14.44                                                       & 11.15/18.94                                                       & 21.44/26.02                                                           & 17.80/25.38                                                              & -/-                                                                 & -/-                                                                    \\ \hline
\textbf{Mintaka} & 3.72/\textbf{11.72}                                                         & 4.86/\textbf{12.79}                                                          & 6.93/\textbf{16.58}                                                       & 12.15/\textbf{20.51}                                                       & 23.87/\textbf{27.88}                                                           & 19.23/26.38                                                              & -/-                                                                 & -/-                                                                    \\ \hline
\multicolumn{9}{c}{\textit{Mintaka (One-hop, English)}}                                                                         \\ \hline
-                & 0/4.70                                                             & 0/4.41                                                              & 0/4.71                                                           & 0/4.71                                                            & 0.50/6.76                                                             & 17.65/22.94                                                              & 20.88/\textbf{24.71}                                                         & 41.76/\textbf{45.00}                                                            \\ \hline
\textbf{SQWD}    & 2.06/5.88                                                          & 1.76/5.29                                                           & 4.41/8.53                                                        & 7.06/10.00                                                        & 19.71/18.53                                                           & 14.12/14.12                                                              & -/-                                                                 & -/-                                                                    \\ \hline
\textbf{Mintaka} & 9.12/\textbf{10.29}                                                         & 12.65/\textbf{15.29}                                                         & 8.24/\textbf{10.59}                                                       & 14.41/\textbf{15.88}                                                       & 27.65/\textbf{28.24}                                                           & 23.24/\textbf{25.59}                                                              & -/-                                                                 & -/-                                                                    \\ \hline
\end{tabular}
}
\caption{Evaluation results on three KGQA datasets (Hit@1 scores): comparing seq2seq models with and without proposed approach tunned on SQWD, Mintaka and pre-trained seq2seq models without tuning for QA.}
    % \label{tab:full_results_upd}
    \label{tab:full_results}
\end{table*}
